Anisotropic Stiffness and Programmable Actuation for Soft Robots Enabled by an Inflated Rotational Joint

Soft robots are known for their ability to perform tasks with great adaptability, enabled by their distributed, non-uniform stiffness and actuation. Bending is the most fundamental motion for soft robot design, but creating robust, and easy-to-fabricate soft bending joint with tunable properties remains an active problem of research. In this work, we demonstrate an inflatable actuation module for soft robots with a defined bending plane enabled by forced partial wrinkling. This lowers the structural stiffness in the bending direction, with the final stiffness easily designed by the ratio of wrinkled and unwrinkled regions. We present models and experimental characterization showing the stiffness properties of the actuation module, as well as its ability to maintain the kinematic constraint over a large range of loading conditions. We demonstrate the potential for complex actuation in a soft continuum robot and for decoupling actuation force and efficiency from load capacity. The module provides a novel method for embedding intelligent actuation into soft pneumatic robots.

==> old_intro.tex <==
%However, the infinite number of passive and active degrees-of-freedom (DOF) in soft bodies gives a theoretically unbounded collection of possible configurations, resulted from both the internal actuation and external contacts. Shaping the configuration space of the robot to form a useful task space thus becomes the key problem of soft robot design.

%Across a wide spectrum of works that investigate the design of soft robots, utilizing the synergies in the interaction between actuators and the mechanics of the soft body is the key in their design methodology.

%For some works in the field, the design of actuation is the dominant factor in shaping the resulted configuration space. For a generic bending actuator such as the PneuNet actuator, which may be viewed as a minimal continuum robot, the interaction between the inflatable chamber and a strain-limiting layer results in a planar curve tip trajectory and a one-to-one pressure input to body shape mapping. One or two additional symmetrically arranged actuator expands the workspace of a continuum  to 2D and 3D respectively. While having more than three actuators in parallel result in redundancy and does not significantly change the configuration and workspace, the actuation-to-shape mapping changes, with one configuration potentially achieved by multiple combinations of actuator state. While the number of actuators determines the dimensionality of the configuration space, their placement provides a design tool. Introducing asymmetries in actuator and backbone arrangement results in stretching and shrinking of the workspace. Actuators routing that is not parallel to the backbone enables using torsion as an additional design parameter: a helically routed tendon or series of pneumatic chambers result in a constant torsion coupled to the the curvature. More generalized forms of actuator routings, such as those taking a free-form path or featuring irregularly shaped inflatable chambers, allows matching robot configuration to an arbitrary shape, but require optimization based-design approaches to search its complex design space.

%Designing the body structure of the soft robot supplements the active, actuator-oriented approaches by shaping the robot's response to actuation input, while leading to behaviors that passively respond to external contact. Body stiffness is the key design parameter leveraged by the passive approach. Stiffness can be pre-programmed as the local property of the constraining layer, or actively tuned via layer jamming or phase-transition of the backbone material, expanding the configuration space achievable with a small number of actuation input. Variable stiffness via mechanisms such as bi-stable structures enables bifurcating response that adapt to external stimuli. Shaping the stiffness of soft robots may involve joining materials whose Young's modulus differ across magnitudes, necessitating special fabrication techniques to ensure robustness.

%Beyond designing the kinematics of the robot, emerging research looks into sequential actuation, which decouples the phase and frequency of the input signal to that of the robot motion and auguments the configuration space with time as an additional parameter. The methods taken to realize an actuation sequence extend the active and passive approaches presented above: while some works condition the input signal with fluidic logic components and oscillators, others harness the response of actuators of the robot structure to define a motion sequence.

%In this work we seek to bridge the active and passive approach to program kinematics and motion sequence simultaneously. 
